The Quest for Omnioculars: Embedded Visualization for Augmenting Basketball Game Viewing Experiences

Sports game data is becoming increasingly complex, often consisting of multivariate data such as player performance stats, historical team records, and athletes' positional tracking information. While numerous visual analytics systems have been developed for sports analysts to derive insights, few tools target fans to improve their understanding and engagement of sports data during live games. By presenting extra data in the actual game views, embedded visualization has the potential to enhance fans' game-viewing experience. However, little is known about how to design such kinds of visualizations embedded into live games. In this work, we present a user-centered design study of developing interactive embedded visualizations for basketball fans to improve their live game-watching experiences. We first conducted a formative study to characterize basketball fans' in-game analysis behaviors and tasks. Based on our findings, we propose a design framework to inform the design of embedded visualizations based on specific data-seeking contexts. Following the design framework, we present five novel embedded visualization designs targeting five representative contexts identified by the fans, including shooting, offense, defense, player evaluation, and team comparison. We then developed Omnioculars, an interactive basketball game-viewing prototype that features the proposed embedded visualizations for fans' in-game data analysis. We evaluated Omnioculars in a simulated basketball game with basketball fans. The study results suggest that our design supports personalized in-game data analysis and enhances game understanding and engagement.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> [2022 VIS] Omnioculars/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> [2022 VIS] Omnioculars/docs/0_abstract.tex <==
% !TEX root = ../main.tex

%% Abstract section.
\abstract{Sports game data is becoming increasingly complex, often consisting of multivariate data such as player performance stats, historical team records, and athletes’ positional tracking information. While numerous visual analytics systems have been developed for sports analysts to derive insights, few tools target fans to improve their understanding and engagement of sports data during live games. By presenting extra data in the actual game views, embedded visualization has the potential to enhance fans’ game-viewing experience. However, little is known about how to design such kinds of visualizations embedded into live games.
% 
In this work, we present a user-centered design study of developing interactive embedded visualizations for basketball fans to improve their live game-watching experiences. We first conducted a formative study to characterize basketball fans' in-game analysis behaviors and tasks. Based on our findings, we propose a design framework to inform the design of embedded visualizations based on specific data-seeking contexts. Following the design framework, we present five novel embedded visualization designs targeting five representative contexts identified by the fans, including shooting, offense, defense, player evaluation, and team comparison. We then developed Omnioculars, an interactive basketball game-viewing \re{prototype} that features the proposed embedded visualizations for fans' in-game data analysis. 
We evaluated Omnioculars in a simulated basketball game with basketball fans.
The study results suggest that our \re{design} supports personalized in-game data analysis and enhances game understanding and engagement.

} % end of abstract

==> [2022 VIS] Omnioculars/docs/1_intro_v2.tex <==
% !TEX root = ../main.tex

\firstsection{Introduction}
\maketitle

Sports broadcasting and streaming have seen exponential growth in recent years. 
Basketball, for example, is one of the most popular team sports worldwide. 
The NBA league alone averages about 1.4 million viewers per game on ESPN~\cite{espnnba}.
With the advent of novel sensing and image processing techniques,
an increasing amount of live data can now be collected in each NBA game, 
including scores, play-by-play data, and even player trajectories.
This data is released online in real-time and is widely used by sports analysts and coaches to measure the performance of teams, analyze the strengths and weaknesses of players, and make in-game decisions.
Overall, in-game sports data has gradually become indispensable
for professional basketball teams to develop winning strategies~\cite{tian2019use,mcintyre2016recognizing,76ers}. 
Several interactive sports analysis systems have been proposed to help experts consume and analyze in-game data~\cite{seidlBhostgustersRealtimeInteractive,losadaBKVizBasketballVisual2016,zhiGameViewsUnderstandingSupporting2019}. 
However, these systems are not yet readily available for sports fans. 
Subsequently, the information needs of a general audience during a game are largely unmet.

During a game, sports spectators and fans seek different data than expert analysts to facilitate their own game understanding and engagement.
After decades of development, scoreboards or data panels shown on TV are still the dominant method for spectators to obtain data during live games. 
However, presenting data in this way often does not fulfill the individual needs of the audience.
Consequently, perhaps the most common solution for spectators is to look up extra data on mobile devices or separate screens.
For example, basketball fans usually look up live box scores and play-by-play data during a game on the official NBA website~\cite{nba}, ESPN~\cite{espnnba}, or on the respective phone apps.
Such practices, however, distract from the game and limit the amount of in-game data analysis that would increase game understanding and engagement for fans and viewers.
Hence, spectators would greatly benefit from an effective way of analyzing in-game data and information that does not distract from the actual game.

Embedded visualization provides a promising opportunity to satisfy the in-game information needs of spectators, 
as it directly visualizes data within its physical context~\cite{willett2016embedded}. 
Thereby, embedded visualizations eliminate the need for context switching and reduce distractions when looking up data.
Recently, \re{some} commercial~\cite{secondspectrum} and research~\cite{chen2021} systems
have utilized embedded visualizations to augment sports videos (so-called \emph{augmented sports videos}),
providing extra information together with the video in a seamless and engaging manner.
However, all these systems are designed for experts to create augmented sports videos post-game 
and do not support custom visualizations for general audiences during a live game.
\re{In the live game, visualizations need to be simple and allow viewers to consume and analyze data on the fly,}
% Little is known about the design space of embedded visualizations for in-game data consumption, 
which can differ significantly from visualizations in post-game scenarios.
% where visualizations can be fine-tuned outside of the constraints of real-time display and analysis. 
% In sum, 
As such,
it is still an open question on how to best use embedded visualizations to satisfy the in-game \re{data} needs of a sports audience.

% Goal
In this study, 
we aim to fill this gap by exploring the design space of embedded visualizations for live sports in-game data analysis.
We adopted a user-centered design approach throughout the study to answer three questions: 
First, we observe user needs and their workflow through a formative user study to answer \textit{``What data do fans desire in a live basketball game?''}.
Based on survey responses and in-depth user interviews with active basketball fans, 
we identified user needs in obtaining more advanced game data and control over their live game viewing experience. 
Next, we tackle the question of \textit{``What are the design considerations for embedded visualizations in live games, based on user needs?''}, 
by proposing a design framework 
for embedded sports data visualization based on 
\textit{scenario}, \textit{data}, \textit{task}, and \textit{embedded vis}.
We further identify five representative game contexts,
i.e., shooting, offense, defense, player performance, and team comparison,
and develop embedded visualizations for them.
To answer our final question of \textit{``How well do embedded visualizations help users enhance game understanding and engagement?''},
we developed \textbf{Omnioculars}, an embedded visualization \re{prototype} for live TV basketball game viewing \re{to support our design exploration}.
We took inspiration from Harry Potter's Omnioculars for Quidditch games~\cite{harrypotter}, which gives fans the ability to \emph{see everything} during a game.
We created
% integrated Omnioculars into 
a simulated game environment in Unity3D~\cite{unity} based on NBA player tracking data to 
embed live visualizations on top of the simulated game.
We conducted a controlled user study with 16 active basketball fans using Omnioculars.
Users were able to generate distinct game insights with each embedded visualization 
and to utilize Omnioculars to personalize their in-game analysis in our simulated basketball game videos.

In summary, our contribution consists of the first design study on embedded visualization for in-game data analysis of basketball fans.
Second, we propose a design framework to support embedded visualization designs based on game contexts.
Third, we built a simulated game-watching environment and implemented Omnioculars, 
a novel design prototype for showing five embedded visualizations in live basketball game videos based on our design framework.
Finally, we evaluate the merits and limitations of embedded visualization for in-game analysis with basketball fans in a user study.

==> [2022 VIS] Omnioculars/docs/2_related_work.tex <==
% !TEX root = ../main.tex
\section{Related Work}
% In this section, we review visual analysis tools for sports, embedded visualization in sports videos, and personalized game viewing systems.

\para{Visual Analytics for Sports.}
Advances in sensors and computer vision techniques have led to the collection of more fine-grained, high-quality sports data.
Perin et al.~\cite{Perin2018-jh} categorize sports data in visualizations into box score data, tracking data, and metadata. 
Given the highly competitive nature of sports, 
numerous visual analytics systems have been developed to allow domain experts to analyze complex sports data for discovering winning strategies.
For example, SoccerStories~\cite{perinSoccerStoriesKickoffVisual2013} employs a series of soccer-related visualizations, such as in-court trajectories and heatmaps, 
to analyze spatio-temporal data collected in soccer games.
BKViz~\cite{losadaBKVizBasketballVisual2016}, an interactive data exploration tool for basketball games, focuses on the analysis of play-by-play data.
Fu and Stasko~\cite{fu2022supporting} developed interactive visualization systems specifically targeting NBA journalists.
Some sports analytics approaches also leverage machine learning models to predict and extract patterns from the data~\cite{tian2019use,mcintyre2016recognizing,nistala2018using}.
Recently,  with the proliferation of low-cost immersive devices such as Virtual and Augmented Reality (VR/AR),
immersive sports analytics systems have been gaining traction.
Compared to traditional desktop systems, immersive sports analytics systems provide unique benefits, including increased spatial understanding, rich embodied interaction, peripheral awareness, and a large information space~\cite{marriott2018immersive,lin2020sportsxr}.
ShuttleSpace~\cite{ye2020shuttlespace}, a VR-based visual analytics system for badminton data,
enables users to analyze shuttle trajectories from a player's first-person view.
Following their work, 
TIVEE~\cite{chuTIVEEVisualExploration2022} allows experts to explore a large scale of badminton trajectories from both first and third-person views in VR.
While these systems have demonstrated their effectiveness in analyzing sports data, 
most of them are designed for post-game analysis by domain experts, 
leading to a high entry barrier and steep learning curve.
On the other hand, 
compared to post-game analysis systems, 
in-game systems usually can be used by both domain experts and fans to complete lightweight analysis.
However, only a few approaches focus on in-game analysis.
GameViews~\cite{zhiGameViewsUnderstandingSupporting2019}, for example, supports data-driven sports storytelling using in-game data for sportswriters and fans.
Yet, GameViews mainly uses simple visualizations separated from the videos, 
forcing users to switch contexts when watching a game.
We draw on this line of research to develop an in-game analysis tool for \emph{basketball fans},
which features embedded visualizations
% by designing visualizations 
% that are dynamically 
% embedded in videos 
to enable lightweight analytics while retaining an engaging game experience.

\para{Embedded Visualization in Sports Videos.}
Sports data, generally speaking, is inherently associated with its physical environment (e.g., a basketball court).
Visualizing sports data within this physical environment can significantly facilitate the understanding and analysis of the data.
Thus, numerous works have explored visualizing sports data in static court diagrams.
For example, CourtVision~\cite{goldsberry2012courtvision} uses point-based visualizations to present the shot distribution and density for NBA data.
Sacha et al.~\cite{sacha2017dynamic} introduced a trajectory-based visualization system that allows users 
to interactively explore the moving trajectories of soccer players.
To improve the analysis of soccer data, 
Stein et al.~\cite{DBLP:journals/cga/SteinJBSSGCK16} developed a region-based visualization that shows the interaction space of each soccer player.
In recent years, with the rapid development of computer vision and image processing techniques,
visualization researchers have started to directly embed their visualizations into sports videos.
For instance, 
Stein et al.~\cite{steinBringItPitch2018} developed a system to assist soccer game analysis, which automatically extracts and visualizes data from and in soccer videos.
Stein et al.~\cite{stein2018} then extended their work by semi-automatically selecting the presented data based on the game's semantic context.
However, these works mainly target experts for analytic purposes and do not fulfill general spectators' needs. 
More recently, Chen et al.~\cite{chen2021} explored the design space of augmented sports videos and presented VisCommentator, a rapid prototyping tool for authoring augmented racket-based sports videos.
In summary, current work in augmented sports videos focuses on domain experts' analytic and authoring needs. 
Embedded visualizations designed for sports fans are still under-explored. 
In this work, we aim to understand fans' in-game analysis needs and propose a structured design framework for embedded visualization in basketball videos.

\para{Personalized Game Viewing Systems.}
When watching a sports game, 
spectators often look up extra information to satisfy their curiosity, 
deepen their understanding of the game, or generate game insights \re{(as found in our formative study in Sec~\ref{sec:design-requirement-analysis})}.
These information needs vary from person to person, leading to a great demand for personalized game viewing systems.
The most common way fans access additional data is using mobile devices to search the internet when watching the game.
However, this approach inevitably incurs context-switching costs
and significantly impedes an engaging watching experience. 
To overcome this issue, HCI and Computer Graphics researchers have studied interactive game viewing systems 
that enable spectators to look up data while still focusing on the game. %shorten: Human-Computer Interaction 
For instance, Gamebot~\cite{zhiGameBotVisualizationaugmentedChatbot2020} uses a chatbot interface on a mobile app for fans to request and consume game data visualization. 
ARSpectator~\cite{zollmannARSpectatorExploringAugmented2019} uses mobile AR devices to overlay basic game data onto the scene for on-site spectators.
Despite the focus on interaction techniques to access game data, 
the existing work did not evaluate the presentation of game data to facilitate game understanding and engagement.
On the other hand,
E-Sports, such as Defense of the Ancients2~\cite{dota} (Dota2) and League of Legends~\cite{lol} (LoL), are ahead of most traditional sports in providing personalized game viewing experiences due to their interactive, online nature.
In Dota2, for example, the audience can interact with the viewing system to inspect the gaming data (\emph{e.g.}, gold over time) of individual players or the whole team.
Nevertheless, most of these systems only present the data in side-by-side settings, in which the visualizations are displayed in panels separated from the game view.
We envision that embedded visualizations have the potential to seamlessly blend the extra information with the game view, providing a natural, intuitive, and engaging watching experience.
Our work takes a first step towards designing and evaluating personalized game viewing systems with embedded visualizations for traditional sports.

==> [2022 VIS] Omnioculars/docs/3_design_requirements_analysis.tex <==
% !TEX root = ../main.tex

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/process.png}
    \vspace{-6mm}
    \caption{We adopted a user-centered design process throughout the study. We elicited user needs through a survey and interviews, and iterated our designs based on user feedback. } 
    \label{fig:process}
    \vspace{-4mm}
\end{figure}

\section{Formative Study with Basketball Fans}
\label{sec:design-requirement-analysis}

Section~\ref{sec:design-requirement-analysis}, \ref{sec:design-space-exploration}, and \ref{sec:omnioculars} present our user-centered design process towards designing an interactive basketball game-viewing system with embedded visualizations (\autoref{fig:process}).
In this section, we detail a mixed-method formative study using an online survey and
interviews with active basketball fans to better understand the general workflow, pain points, and best practices of fans to acquire desired data during a live game.
% To better understand the general workflow, pain points, and best practices of fans to acquire desired data during a live game,
% we conducted a mixed-method formative study using online surveys and
% interviews with active basketball fans.

% an online survey and followed up semi-structured interviews were conducted.

% To answer our first research question of what data fans desire during a live game, 
% we first conducted a contextual inquiry and followed up with in-depth user interviews to identify gaps in the current workflow. 
% We analyzed the responses to characterize user goals and needs for in-game data analysis and further identified a set of analysis tasks that inform our design.

\subsection{Procedures}
\label{sec:contextual-inquiry}

% To better understand the in-game analysis needs of active fans and the type of data they desire, 
% we followed the format of a contextual query, where researchers observe a user perform tasks in a live setting and record the observation instantly~\cite{hartson2012ux}.
% Due to the limitation posed by COVID-19, we designed an online survey to collect contextual responses,
% which was tied to a specific game viewing experience and required respondents to record their observations in real-time.

We first used an online survey to collect initial feedback on basketball fans' data needs while watching live games.
We analyzed survey responses to understand fans' in-game data analysis behaviors
and to inform the questions of the follow-up interviews (\autoref{fig:process}).

\para{Online Survey.}
The game-watching experiences survey \re{(Appendix A)}
% had 6 closed questions and 13 open questions, which 
asked about fandom levels (\emph{novice}, \emph{casual}, \emph{engaged}, and \emph{die-hard} fans), game watching frequency, \re{and in-game data analysis records}.
We asked respondents to watch a live basketball game 
and record three moments when they wanted to look up additional data. 
We advertised the survey using university mailing lists
and only collected responses from casual fans and above.
In total, we gathered 14 responses (R1-14; M = 10, F = 4; Age: 18 - 45) \re{and 40 records of their data-seeking moments when watching a live game}.
All respondents are NBA fans (4 casual, 6 engaged, and 4 die-hard fans).
% \re{Survey details can be seen in Appendix A.}
% The respondents contributed 40 in-game data analysis records.

\para{In-depth Interview.}
We then interviewed six fans from the survey respondents (I1-6; 4 die-hard and 2 engaged fans) who expressed interest in the survey. 
Among them, five have been NBA basketball fans for over ten years.
We conducted the interviews remotely using Zoom in two parts (Appendix B).
We first asked respondents about their overall game viewing experiences 
and data analysis behaviors in recent games they watched, 
including occasions they looked at data and whether the data was helpful and engaging.
% with a focus on the 
% We asked them to compare their game-watching experience between on-site game viewing, TV streaming, and highlight game videos, 
% with a focus on the useful form of information and visual effects in each medium,
% and to describe the data they consume during the live game with examples.
We then asked them to watch three video clips selected from a 9-minute post-game highlight video of an NBA regular-season game\footnote{Golden State Warriors vs. Cleveland Cavaliers, 2015} and think aloud about what game insights and data they observed and wanted to see.
Each clip consisted of two to four plays for about 30 seconds and collectively covered a diverse range of gameplays, 
including offense strategy, a player's highlight (a layup with a foul), defense performance (a block), or clutch time.
The clips also included video effects to augment certain gameplay, such as replays from different angles, showing a player's box score on the screen, etc.
The interviewees contributed 63 in-game data analysis records on the three clips. \re{No further interviews were conducted as saturation was met in the analysis.}
% No compensation was provided. 

% Each observation contained 
% \textit{when} they wanted to see additional data, 
% \textit{what} data they wanted to see, 
% \textit{why} they wanted to look up the data, 
% and \textit{how} they got these data. 

\para{Analysis.}
We performed a reflexive thematic analysis~\cite{braun2019reflecting} on the survey and interview data. % analysis records.
Three authors began coding separately on the 40 survey records to create sets of plausible codes, 
and through later discussion and affinity diagramming with another author,
agreed on a single coding scheme.
Then the lead author finished the coding on the remaining records collected from the interviews.
% Other game experience insights were obtained from interview notes.

% We analyzed the 40 contextual records using Affinity Diagramming, 
% which is a common method to generate hierarchical categories and induce patterns from dissimilar qualitative data.
% Four authors used Miro board~\cite{miro} to categorize the 40 contextual records into \emph{User Goals (Why)}, \emph{Contexts (When)}, and \emph{Data (What)}.
% Each response was posted as a separate sticky note and all coders moved notes around to group similar themes. 
% Similar groups were further categorized to form larger groups until all coders reached a consensus.
% \zt{reference:  
% Two members of the research team began open coding separately to create sets of plausible codes, and through later discussion and affinity diagramming, agreed on a single coding scheme. 
% The themes were conceptualized based on the codes to examine the complex web of
% factors underlying the process of knowledge communication. The survey responses were
% analyzed using Microsoft Forms to understand viewers’ consumption behaviors and inform the
% interview questions for the viewers.}

\subsection{Findings and Discussions}
\label{ssec:survey-interview-findings}

% From the user experience inquiry, 
We present findings on fans' motivation, workflow, and pain points of performing in-game data analysis.

\subsubsection{Practices of Watching Live Basketball Games}

Overall, most of the respondents watched NBA games at least once per week (4 watched 3 games per week, 9 watched 1-3 games per week, 1 watched less).
12 of them followed a team or a player in the NBA league.
All six interviewees watched 1-3 NBA games per week, 
mainly to follow their favorite players. 
As for the game watching media,
the interviewees explained that while watching games on-site is engaging and exciting for all fans, 
they mostly watch live streams for convenience and economic reasons. 
When asked to compare their game-viewing experience between live streams and highlight videos, 
interviewees expressed that 
they preferred to watch live streams over highlights. 
One key reason is that highlight videos do not present the flow of the game. 
Although highlight videos usually provide additional visual effects, 
such as play breakdown or embedded data overlays, 
fans cannot observe how the game developed to the current moment and feel \textit{``it shows no rhythm of the game''} (I4). 
In summary, compared to on-site watching and highlight videos,
live streaming is the favorite game watching medium among fans \re{we surveyed}.

% In particular, they focused on their favorite player's movement, performance, and decisions. 
%\textbf{This finding further highlights the need to take contexts into account to design embedded visualization for in-game data analysis}. \jb{last sentence unclear, why does this finding highlight that? Maybe the following sentence:}
% This finding further highlights the \textbf{importance of following a game over time, and for fans to be able to decide \emph{when} to see additional information}, i.e., the context of embedded visualizations for in-game data analysis. 
% We further asked fans to comment on the data and visual effects they found useful in their game viewing experiences. 

\subsubsection{Seeking Data in Various Contexts During Live Games}
\label{ssec:data_context}

% Seeking data while watching a live game is a common behavior among fans.
Seeking data while watching a live game \re{was a common behavior among fans we surveyed}.
While watching a game,
all \re{14} respondents in the survey expressed interest in looking up game data; % while watching a game.
all six interviewed fans confirmed that they 
always look up game stats to complement the viewing experience.
Based on our analysis of the records, 
a context in which a fan seeks data while watching a live game
can be characterized by a \Scenario{}, \Data{}, and \Task{}.
Specifically, 
in different scenarios (When), 
fans seek different data (What) to accomplish different tasks (Why):
% deepening their understanding of the game and increasing the engagements of the watching experience.

\para{Fans seek data in three typical \Scenarios{} (When)}.
First, fans often look for data at \emph{\textbf{specific game times}}, such as before the game, during halftime, or in the last quarter.
These specific game times are defined based on the rules of the sport, like basketball, and thus usually have special meanings.
 %(e.g., \textit{``Right before half-time''}) tip-off'', ``timeout, half-time, or post-game''}) and in the last quarter of the game (e.g., \textit{``In the 4th quarter, especially before the clutch time''}).    
Second, fans seek data when observing \emph{\textbf{a game event}}.
These events include seeing a game stat, a game action, or the appearance of a new player, \textit{``D. Rose made an and-1 play in the 2nd quarter''} (R8).
Third, when \emph{\textbf{multiple repetitive game events}} happen,
fans sometimes want to seek data to evaluate a player's or team's performance related to this specific type of game event, \textit{``Thunder is missing a lot of 3 pointers''} (R5).

\para{Fans seek two types of \Datap{}  (What).}
Based on the survey and interviews, the data sought by the fans can be divided into two types, inspired by Perin et al.~\cite{Perin2018-jh}.
First, \emph{\textbf{game data}} are directly collected from games, 
including box score, \textit{``foul number of Embiid''} (R4),  
tracking data, \textit{``the usage of this particular play''} (R9), %``the percentage when there is no defender in the front''}, 
and video data. %(\textit{``a comparison between offensive and defensive fouls in a similar situation.''}). 
The game data sought by the fans can range from a single game, to multiple games, or an entire career.
Second, \emph{\textbf{metadata}} includes data beyond games, such as ranking, player background, and news. 
% Unlike Perin et al.  categorized data used in sports visualization designs~\cite{Perin2018-jh}, our data categorization is derived from the data desired for in-game analysis by fans.  
% We categorized data types consumed during the game from 40 contextual responses of \textit{``What data do fans want to see during the game?''}. 

\para{Fans seek data to finish three \Tasks{}  (Why)},
ultimately generating insights to deepen their understanding of the game.
Inspired by  Brehmer and Munzner~\cite{brehmer2013multi,munzner2014visualization},
we summarized three typical tasks that the fans perform with data during a live game.
First, fans seek data to \emph{\textbf{identify}} the performance of players or teams.
For example, a respondent replied, \textit{``I was wondering whether he was getting a triple-double''} (R4). % (new record). 
In addition to looking at the data of a specific player, fans are also interested in
the data of the whole team, such as the moving trajectories of a team to 
``\emph{understand the offensive and defensive strategies}'' (I3).
Second, fans often need data to \emph{\textbf{compare}} the in-game performance of a player or team 
to others' in-game performance or to their historical performance.
For example, a respondent replied, 
\textit{``I want to know how many assists our team makes compared to other teams''} (R5).
% Besides, fans also want to compare the in-game data of players or teams to their historical data.
Five interviewees also provided that they wanted to compare a player's in-game performance
to their average performance to evaluate the consistency.
% \textit{``To know that whether is the team normal performance to miss a lot of 3 pointers.''} 
Third, fans usually seek data to \emph{\textbf{summarize}} the performance of players or teams.
% at particular game moments, such as during timeouts or in the fourth quarter. 
Compared to the other two tasks, as pointed out by Brehmer and Munzner~\cite{brehmer2013multi,munzner2014visualization},
% simply looking up a game stat,
the summarize task often involves a deeper analysis of the data, such as overviewing the game and observing patterns, 
deriving the cause of the performance, 
and speculating on possible outcomes. 
Representative responses include \textit{``to have a quick understanding of both teams so I know what to expect in the match''} (R10) (overview \& possible outcome) and 
\textit{``to understand what causes the score difference between two teams''} (R3) (cause of the performance). 

\subsubsection{Pain Points of Seeking Data in Watching Live Streams}
While seeking data \re{was} common among basketball fans,
the data acquisition process in practice remains hindered by current technologies.
According to the survey, the main method of acquiring data is through websites or mobile apps (30 out of 40).
% while only in a few (\zt{num}) case the respondents can obtain data through the arena or TV scoreboard.
In the interviews,
the fans further detailed that they access websites (ESPN~\cite{espnnba}, NBA~\cite{nba}, or Reddit~\cite{reddit}) 
on the phone or on a separate screen to regularly track box score data or team standing. 
Such practices reflect several issues in the live game-watching experience:

\para{Data provided by live streams lack diversity.}
The interviewees agreed that 
most information available on live streams, such as game stats and timers, 
was useful.
However, they also confirmed that the information provided by the live streams is not diverse and sufficient enough, e.g., \textit{``usually they are not sufficient, only showing a matrix of all player names and scores (I2)''}.
Some information that the interviewees would love to have is usually absent in live streams, 
such as seeing all box scores and lineups information, or comparing shooting performance by zones.
% explaining play sets or offense strategies, or highlighting the player formation (e.g., weak side vs. strong side).
This is the main reason that fans search websites to obtain extra data while watching live games.

\para{Data provided by live streams lack controllability.}
Interestingly, although live streams can provide some basic box score data (like game stats and timers),
the interviewees still will check this data on the website regularly, 
\textit{``Right now, on a separate screen, I can look at the full box scores to get an updated impression of the players''} (I4).
%\textit{``I do like right now [on a separate screen] I can look at the full box scores to keep updated my impression of the players''} (I4).
This practice reflects that when watching live games,
fans need not only sufficient data but also the ability to control when and what data to show.
This finding also links to our characterization that users seek different data in various contexts (Sec.~\ref{ssec:data_context}).

\para{Data provided by websites are separated from the game videos.}
Unsurprisingly, the interviewees complained that looking up data on the phone or a separate screen reduces the engagement of the game watching experience as it introduces numerous context switches between the game videos and websites.
For example, \textit{``in a live game there’s a lot going on and likely I missed some events [when looking up data]''} (I1).
Thus, interviewees would like a more intuitive method to present the data directly within the game videos.

\subsection{Summary}

Our \re{formative study} found that live streams \re{were} the favorite watching medium for basketball fans \re{we interviewed}.
While watching live games,
fans seek different types of data in different scenarios for different tasks. 
However, current live streams \re{fall short in fulfilling fans' diverse data needs,} 
% cannot fulfill fans' data needs as streams lack data diversity and controllability,
forcing fans to look up data on separate screens (phones or monitors),
which reduces the engagement in watching games.
To tackle these issues,
we propose to \re{embed visualizations into live game videos to present data in-situ and support in-game data analysis.}
% develop an interactive game watching system that features embedded visualizations to present the data seamlessly within game videos.

==> [2022 VIS] Omnioculars/docs/4_design_framework.tex <==
\section{Design Space Exploration}
\label{sec:design-space-exploration}

To answer our second research question of how to design embedded visualizations for fans' in-game data analysis, 
we first developed a design framework based on the formative study findings (\autoref{fig:design_framework}).
With this framework, we then identified 20 contexts from the \re{records of fans' in-game data seeking moments}. By walking through these design contexts using design mockups with the six interviewees,
we prioritized five contexts to be implemented in our \re{prototype}. 

% This section presented our design framework, iterative process, and design details.
% to explore the design space.
% and exemplify 20 scenarios with design sketches. 
% By walking through these design scenarios with the target users, 

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/Design_Framework.png}
    % \vspace{-6mm}
    \caption{Design framework for context-driven embedded visualizations.} 
    \label{fig:design_framework}
    \vspace{-3mm}
\end{figure}

\subsection{Design Framework}

% Based on the findings of our formative study, % with basketball fans' game viewing experience, 
Based on the data-seeking contexts we summarized in Sec.~\ref{ssec:data_context},
we propose a context-driven design framework for embedded visualizations for in-game data analysis (\autoref{fig:design_framework}). 
The framework scaffolds the relationship between four design aspects -- 
``\emph{In a certain \Scenario{}, the user performs a \Task{} on \Data{} using \EmbeddedVis{}}'':

\begin{itemize}
    \item \Scenario{} describes the background of fans' data analysis behaviors.
    Three design elements can be used to describe a scenario that drives a fan's data need:
    \Target{} \emph{target} (team or player),
    \Event{} \emph{event} (any game event that is happening), %such as make a shot, or commit a foul; 
    and \Time{} \emph{time} (a specific moment or a duration). %, such as the last two minutes, or at the current time. 
    % Any game scenario that drives a fan's data need can be described with these three elements. 
    For example, \textit{``When Joel Embiid fouled''} describes a player (target) with a foul (event) at the current time (time);
    \textit{``When we have been making strides with offense for a streak of time in the game''} describes a team (target) make shots (event) over a certain period (time). 

    \item \Data{} that is of interest to fans can be collected in-game or beyond games.
    For embedded visualizations, we focus on in-game data and exclude metadata.
    Thus, the data types to be considered include 
    \Boxscore{} \emph{box scores} (game summary scores), 
    \Tracking{} \emph{tracking data} (like player positions), 
    and \Video{} \emph{video}.
    Different data can be further combined to specify advanced stats, 
    such as \textit{``the lineup's plus-minus''} or \textit{``the shot percentage of \#30 when there is no defender in the front.''}

    \item A \Task{} is performed on game data by fans to generate insights about players or teams,
    including \Identify{} \emph{identify} (on a player or team), 
    \Compare{} \emph{compare} (between players or teams), 
    and \Summarize  \emph{summarize} (among players or teams).
    
    \item \EmbeddedVis{} can present in-game data directly in videos to support fans performing in-game data analysis naturally.
    Prior research~\cite{chen2021} systematically studied the design space of augmented sports videos
    and summarized the embedded visualizations used in augmented videos to present sports data.
    We follow their design space with a focus on embedded visualizations for basketball,
    and identified five relevant graphical marks and basic visual elements:
    \Point{} \emph{point}, 
    \Line{} \emph{line}, 
    \Area{} \emph{area}, 
    \Label{} \emph{label}, 
    and \Panel{} \emph{side panel}. 
    These basic visuals can be composited to construct embedded visualizations in basketball game viewing.

\end{itemize}

This design framework helps designers 
identify fans' in-game data analysis contexts 
by specifying the \Scenario{}, \Data{}, and \Task{}.
Such a context captures the fan's specific requirements for in-game data analysis at a given moment.
Once a context is identified, the designer can then focus on the design of embedded visualizations 
by composing the five basic visuals,
thereby ensuring the embedded visualizations are developed based on and can satisfy the fan's analysis needs.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/Design_Context.png}
    % \vspace{-6mm}
    \caption{We developed five embedded visualization designs based on our design framework and the five prioritized contexts in Sec.~\ref{sec:scenario-walkthrough}.} 
    \label{fig:design_context}
    \vspace{-3mm}
\end{figure}


\subsection{Design Context Walkthrough}
\label{sec:scenario-walkthrough}

Following our design framework,
we identified 20 design contexts from 103 
\re{records of in-game data seeking moments}
% in-game data analysis records 
in the formative study 
% (40 and 63 from surveys and interviews, respectively) 
\re{by grouping similar records and summarizing representative contexts}.
We created 20 design mockups to demonstrate the contexts (Appendix C) and 
% we proposed and sketched a few variations of embedded visualizations by composing the five basic visuals.
% Next, we 
walked through them with 
%walked them through %the 20 designs and proposed visualizations 
%with 
the six fans in follow-up interviews.
Based on their ratings of importance, we prioritized five contexts that drove the design of five embedded visualizations in our \re{prototype} (Fig.~\ref{fig:design_context}).

\begin{itemize}
    \item[\textbf{\texttt{C1}}] \texttt{\textbf{Shooting}} -- A player shoots (\Scenario{}), 
    and the fan wants to identify and compare (\Task{} \Identify{}\Compare{}) the player's box score (\Data{}). 
    % We proposed showing shot performance box score as a label on top of the player. 
    % During the design walkthrough, 
    Fans found this context useful and suggested avoiding information overload by only showing the most important stat based on player and location. 
    % Therefore, it is not necessary to show the 2-point stats if the shooter made a 3-point shot. 
    % This scenario led to the Shot Label design in Omnioculars.


    \item[\texttt{\textbf{C2}}] \texttt{\textbf{Offense}} -- The offense team runs a play (\Scenario{}), 
    and the fan wants to identify and compare (\Task{} \Identify{}\Compare{}) the players' movement (\Data{}). 
    % We proposed to show the movement with trails (line) and highlight the ball handler's position with a circle (point). 
    Fans commented that this context is very useful to follow the ball and understand the play better, especially for tracking off-ball players and identifying open shot opportunities. 
    % This scenario led to the Offense Trajectory design in Omnioculars.

    \item[\texttt{\textbf{C3}}] \texttt{\textbf{Defense}} -- The defense team defends well/poorly (\Scenario{}), 
    and the fan wants to identify (\Task{} \Identify{}) the defense scheme (\Data{}). 
    % We proposed to highlight the players' defense zone  with circles (area), 
    % linking the defender to his offensive player to show the distance (line). 
    Fans commented that 
    % the defense scheme frequently changes so showing individual defense zones will be overwhelming. However, highlighting the ball defender and distance to the ball is 
    this context helps identify the effective defenders and track how defensive focus is changing. 
% This scenario led to the Defense Form design in Omnioculars.

    \item[\texttt{\textbf{C4}}] \texttt{\textbf{Player Performance}} -- A player has made/missed shots (\Scenario{}), 
    and the fan wants to compare and summarize (\Task{} \Compare{}\Summarize{}) the player's shot performance by zones (\Data{}).
    % We proposed to show an embedded heat map of the player's average shot percentage by zones (area) with the shot locations (point). 
    Fans found this context helpful for evaluating a player's game performance in more detail with direct reference to their average performance.
    % In terms of usability, we were concerned about the potential visual clutter caused by the large colored areas. 
    % Fans said they would use this scenario less frequently, 
    % but it is still useful during the game break, such as during a foul, dribbling, or out-of-bound shot.
    % This scenario led to the Shot Chart design.

    \item[\texttt{\textbf{C5}}] \texttt{\textbf{Team Comparison}} -- At the clutch time (\Scenario{}), 
    the fan wants to compare and summarize (\Task{} \Compare{}\Summarize{}) team stats (\Data{}). 
    % We proposed to show the key team stats comparison on a side panel and highlight the strengths and weaknesses of each team with visual encoding. 
    Fans commented instant access to this data is very convenient during the game break. 
    % This scenario led to the Team Panel design.
\end{itemize}



% \para{Scenario 5 -- Replay.} A player made a beautiful shot, and the fan wants to see a slow-motion replay. We proposed to have a side panel showing the replay with different angles and slow motion, with the ability to overlay box score (label). Fans found this scenario useful as they would already rewatch some highlights during the game break. 
% We decided not to implement this scenario because video replay is not the focus of our study. 

% \begin{figure*}[tb]
%   \centering
%   \includegraphics[width=\linewidth]{images/EmbeddedVis.png}
%   \vspace{-6mm}
%   \caption{Five embedded visualization designs in Omnioculars.}
%   \vspace{-6mm}
%   \label{fig:embeddedvis}
% \end{figure*}


==> [2022 VIS] Omnioculars/docs/5_Omnioculars.tex <==
% !TEX root = ../main.tex

\section{\Omnioculars{}}
\label{sec:omnioculars}

Building upon our design space exploration in Sec.~\ref{sec:design-space-exploration},
we present Omnioculars, 
an interactive embedded visualization \re{prototype} for live game data analysis for fans.
Omnioculars consists of three main components:
a game simulator, embedded visualizations, and interactions.
% We describe each component in detail.

% design goal is to provide personalized data access through context-driven embedded visualization for live game analysis. 
% Five embedded visualizations were designed to support five primary contexts identified in Sec.~\ref{sec:scenario-walkthrough}.
% Below, we describe the implementation and design considerations in detail. 
% \zt{we may need a figure to show the components of Omnioculars}

\subsection{Game Simulator}
\label{sec:data-source}

Ideally, Omnioculars should be built on top of live stream TVs 
as a third-party game viewing system
to enhance the real-world watching experience.
However, we decided to develop 
Omnioculars on top of a game simulator instead of real-world broadcasting videos, considering two aspects:
On the one hand,
implementing Omnioculars based on publicly available broadcasting videos is extremely difficult.
First, the data that can be extracted from broadcasting videos is limited
due to the reduced frame rate and low resolution.
Second, rendering embedded visualizations into broadcasting videos is challenging 
as the camera parameters of these videos are usually not made public.
Third, broadcasting videos often switch between cameras and insert replays,
reducing the controllability of Omnioculars.
% which are uncontrollable for a third-party game viewing system.
On the other hand,
our goal is not to develop Omnioculars as a fully functional system used in real-world scenarios
but as a design probe~\cite{DBLP:conf/chi/HutchinsonMWBDPBCEHRE03} to explore the notion of using embedded visualizations to improve game viewing experiences.
% interactive game viewing system with .
% Achieving a high-quality game simulation is extremely technical-challenging and expensive (e.g., NBA 2K games\cite{nba2k} were developed by a large team of engineers and cost millions of dollars) and this is not our focus.
To gain feedback on our design without being bogged down by the aforementioned engineering challenges,
we use a game simulator as the system's basis, % of Omnioculars,
thereby obtaining richer data, better rendering results, and controllability.
Please note that the aforementioned challenges can be tackled 
once the source video streams 
and sensing data from the live game collected by the TV companies and NBA league
are available.

{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{table}
    \centering
    % \vspace{-0.5mm}
    \caption{The required data for the game simulator.}
    \label{tab:data}
    \vspace{-0.5em}
    \begin{tabularx}{\columnwidth}{p{2cm} p{5.7cm}}
    \toprule
    
    \textbf{Type} & \textbf{Description} \\ \midrule
    Tracking Data & The players and the ball's position over time. \\ \hline
    Event Data & The game events, each event is described by its time, player, action, and outcome. \\ \hline
    Shot Locations & The position of each shot event. \\ \hline
    Box Score & Team and player statistics of the game. \\ \hline
    Player Zoned Shot  \%  & Player's detailed shot percentage by shot locations grouped into zones.   \\ \hline
    League Average Zoned Shot \% & The NBA league's average shot percentage by shot locations grouped into zones.\\
	\bottomrule
\end{tabularx}
\vspace{-4mm}
\end{table}
}

The game simulator is implemented using Unity3D~\cite{unity},
with a 3D basketball arena and 10 player models (\autoref{fig:teaser}).
To simulate a basketball game, we adopt a data-driven strategy.
Specifically, the simulator takes a set of spatio-temporal data as the input
and outputs a virtual basketball game 
by moving the players and triggering events based on the data.
Table~\ref{tab:data} shows the required data in our current implementation.
Overall, 
as suggested in the user study (Sec.~\ref{sec:game-simulation}),
the simulated game was perceived as comparable to an actual game in terms of acquiring game insights by the users.

\subsection{Embedded Visualization Designs}
We iterated over each of our visualization designs with two fans we interviewed.
%Each visualization was designed and iterated with 
% user feedback from 
%two fans we interviewed. 
Both were die-hard fans with substantial basketball knowledge and game viewing experiences. Therefore, we considered them to be domain experts and asked for feedback on our visualization designs.


\subsubsection{Shot Label} 
% \vspace{-5mm}
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/EV1-HD-Reversed.png}
  \vspace{-5mm}
  \caption{Shot Label shows (a) static outcome and (b) dynamic percentage.}
%   \vspace{-2mm}
  \label{fig:ev1}
\end{figure}

\noindent
In \texttt{C1 Shooting}, 
we identified that fans want to see the shot performance of the shooter before and after shooting to predict and evaluate the shot outcome,
and compare the shooter's shot percentages to their average or others' performance. 
We propose a \ShotLabel{} that consists of two components:
1) a static label with the shooter's shot outcome at the shot location (\autoref{fig:ev1}a)
and 2) a dynamic label showing the player's shot percentage based at their current location (\autoref{fig:ev1}b).

The static 
% shot attempt 
label is shown at the shot location after a player shoots and is visible for 5 seconds and
presents the shot outcome, the shooter's game, and the average shot percentage with bar charts. 
This allows fans to get a quick comparison of the shooter's own in-game performance without interfering with the continuing game. 

The dynamic label shows the shooter's average shot percentage based on the location above their head and moves with the player. 
This supports comparing the player's shot performance among their team and instantly evaluating the player's shot opportunity based on location. 
The dynamic shot percentage is obtained from one of the seven shot chart zones (see Fig.~\ref{fig:ev4}). 
To support direct visual comparison, 
the label is color-coded to compare the player's shot percentage to the league's average, 
colored in red (hot) if above and in blue (cold) if below. 
The dynamic label supports fans to compare the shooter's shot percentage to other players, 
such as evaluating if the shooter is shooting from their hot spot, and the quality of shot selection.

Alternatively, our original design had a label pop up right after a shot
and move with the shooter for a few seconds, showing the score and shot percentage of the shooter.
However, fans' feedback suggested that dynamic labels with dense information are difficult to read and showing a player's shot outcome as the player moves into the next play does not help with game analysis. 
Thus, we abandoned this design.
%This design thus was abandon.

% We designed the label to move with the player and stay for a few seconds, so that fans can read the stats as the game continues.
% final design

\subsubsection{Offense Trajectory}

\setlength{\intextsep}{0pt}%
% \setlength{\columnsep}{6pt}%
\begin{wrapfigure}{R}{0.22\textwidth}
	\centering
	\includegraphics[width=0.22\textwidth]{images/EV2-HD.png}
	 \vspace{-4mm}
	\caption{Offense Trajectory}
	 \vspace{-2mm}
	\label{fig:ev2}
\end{wrapfigure}
% \setlength{\intextsep}{12.0pt plus 2.0pt minus 2.0pt}%
% \setlength{\columnsep}{10pt}%

In \texttt{C2 Offense},
fans were eager to use visualization to track the playset and spot open shot opportunities from the off-ball players.
Our \Offense{} design (\autoref{fig:ev2}) shows the offense players' trails and highlights the open space around an offense player with a circle underneath the player (area). 
The radius of the open space is drawn based on the player's distance to the closest defender and changes dynamically to reflect the interaction between the offense and defense team. 
We also color the ball handler's open space in red to guide the viewer's attention. 
Fans can identify the play run by the offense team through the trails, 
and easily tell the speed and rotation of the players. 
The open space circles reveal how the defense team reacts to the play and help fans immediately spot open shot opportunities (larger circles). 

% design iteration
Before finalizing the design, we iterated on the design 
by encoding other useful tracking data, 
such as speed measurement, player role, and distance to other players. 
User feedback suggested that encoding speed and player roles does not provide much value as a player's speed changes constantly 
and does not represent the actual moves of the player. 
The differentiation of player roles also became less prominent in modern basketball games. 
However, encoding the distance to the defense player was deemed very useful for fans to track the execution of the play.
We thus kept this encoding.

% In the first design, 
% we highlighted the trajectory of offense players (line), 
% and the position of the ball handler (point). 
% To avoid visual clutter, we chose a pale color and only showed the trajectory for 2 seconds.
% While this design fulfilled the first design requirement of tracking the playset, 
% it did not provide fans with deeper insights on the interaction of the play run, 
% such as how the defense reacts and how each individual role develops. 

\subsubsection{Defense Form}
\vspace{1mm}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/EV3-HD.png}
  \vspace{-5mm}
  \caption{Defense Form shows (a) ball defender and (b) defensive focus.}
%   \vspace{-2mm}
  \label{fig:ev3}
\end{figure}

\noindent
In \texttt{C3 Defense}, 
fans wanted to identify the defense scheme and key defenders, 
and track the change of defenders when a switch happens. 
The \Defense{} 
highlights the key defenders by tracking the distance between the defenders and the ball handler 
(\autoref{fig:ev3}a). 
When a defender is within $6 \ft$ of the ball, that player is marked as the ball defender (dark blue) and connected to the ball handler with a line. 
The defender is marked as a helper (blue) if within $12 \ft$ of the ball. 
When multiple defenders are identified as key defenders on the strong side (the ball handler's side of the court), the enclosed area is colored to highlight the region of defensive focus (\autoref{fig:ev3}b). 
Fans can evaluate the defense scheme 
% and dynamic change 
from these visual marks without being overwhelmed.

% design iteration
An alternative design was to highlight the position of all defensive players (point) 
and color the enclosed region (area) to achieve the goal of tracking the defense scheme and transformation. 
However, this design did not specify the key defenders, 
including the ball defender and helpers on the strong side. 
Furthermore, the large enclosed area can cause visual clutter,
and does not represent the actual defense focus, 
as the further away the defense players are from each other, the less of a threat they are. % fewer threats they have in the space in between. 
% The large colored area also caused visual clutter.
% We iterated on simplifying the visual presentation based on the user goals. 
Instead of highlighting all defensive players, 
our final design focuses on
drawing user attention to the effective defenders and showing the defensive focus of the enclosed area between key defenders.     

% final design


\subsubsection{Shot Chart}

In \texttt{C4 Player Performance}, 
fans valued the benefit of using embedded visualization to compare the shooter's shot performance in game to their own seasonal average in more detail. 
\begin{wrapfigure}{r}{0.21\textwidth}
	\centering
	\includegraphics[width=0.21\textwidth]{images/EV4-HD.png}
	 \vspace{-6mm}
	\caption{Shot Chart}
	 \vspace{-0mm}
	\label{fig:ev4}
\end{wrapfigure}
We designed \ShotChart{} to have two components, 
a heat map and a player panel (\autoref{fig:ev4}). 
The heat map shows the player's seasonal shot percentage by zones (detailed in Sec.~\ref{ssec:otherdesigns}).
The areas are color-coded by the comparison to the league shot percentage average, 
from dark blue ($\leq -10\%$), blue ($\leq -5\%$), yellow ($\pm 5\%$), orange ($\geq 5\%$), and red ($\geq 10\%$). 
We also visualize shot attempts and locations with 3D basketball icons on the court to represent made (colored ball) and missed shots (black ball).
The heat map design allows fans to evaluate the shooter's detailed game performance directly within the game contexts, such as observing whether the shooter made shots in their hot zone or comparing the shot number in each zone. 
The player panel is shown on the courtside to show player box score stats, 
providing a complete picture of the player's game performance besides shooting.

% design iteration
% We iterated on the data to be shown in the shot chart. 
% As current shot charts on sports websites during the game only show the shot attempts as points on the court, 
% fans were eager to get more details of the shot performance.
% There are different design options, including showing the team or player's own shot average, and number of zones to be segmented (discussed below in ``Other design considerations''). 
% As most fans are more concerned about individual players and evaluate their favorite players' in-game performance, we defaulted to show the shooter's shot chart.

\subsubsection{Team Panel}

\begin{wrapfigure}{R}{0.21\textwidth}
	\centering
	\vspace{-1mm}
	\includegraphics[width=0.21\textwidth]{images/EV5-HD.png}
	 \vspace{-5mm}
	\caption{Team panel}
	 \vspace{-0mm}
	\label{fig:ev5}
\end{wrapfigure}

Based on \texttt{C5 Team Comparison}, 
\TeamPanel{} is designed to provide an overview of team stats and compare team performance. 
As shown in~\autoref{fig:ev5}, 
the panel is shown at the courtside to allow instant look-ups without losing sight of the game in the front. 
Each stat label uses the color of the team with the better performance,
%is colored in the team color that has better performance, 
such as blue for 3 Pointers (Warriors have a higher shot percentage). 
The bars for each shooting stat (Field Goals, 3 Pointers, and Free Throws) are colored based on the shot percentage compared to the league's average using the same colors as Shot Chart. \re{For example,} Cavaliers have a lower 3PT shot percentage than the league's average and are coded in dark blue.
% compare to existing vis
Showing a team stats comparison on a panel is common in current TV streaming services during breaks, but it usually requires cutting away from the court view.
%but they usually show it as a change of view. 
Instead, our team panel design is always-on, without interfering with the game and thereby providing an effective direct comparison through colors.

\subsubsection{Other Design Considerations} \label{ssec:otherdesigns}

\para{Color Usage.} 
Our color encoding of shot percentages uses blue to red and is based on the convention of basketball analysis, where red indicates a hot hand (good performance), and blue indicates cold (bad performance). Similarly, Offense Trajectory uses a color scheme of reddish tones to indicate offense strengths, while Defense Form uses blue tones to show defense efforts.

\para{Shot Percentage Threshold.} 
We use the NBA's official shot charts~\cite{nbastats} and color palette to compare player and league shot percentages. 
%The comparison thresholds in Shot Chart are based on the NBA's official shot charts~\cite{nbastats}. We used the same threshold and color palette to compare player and league shot percentages. 

\para{Defense Distance Threshold.} 
We define the effective defender as being within $6 \ft$ of the offense player based on the definition of an open shot~\cite{lucey2014get}.
% http://www.yisongyue.com/publications/ssac2014_open_shot.pdf
The threshold decreases to $3 \ft$ if the offensive player has passed the defender, as a threat from the back is low. We double the threshold ($12 \ft$) for helpers as an approximation to indicate the strong side range as  there is no accurate definition for defensive helpers.

\para{Shot Chart Zones.} 
We segmented the shot chart into seven zones, including rim (within $8 \ft$), mid-range (left/right-wing), corner three (left/right), and 3-point range (left/right). We aggregated the 19 zones in the NBA shot chart~\cite{nbashotcharts} to strike a balance betwen visual complexity and usefulness. 
% https://www.nba.com/clippers/news/clippers-shot-chart-analysis

\subsection{Interactions}

While the five embedded visualizations can be displayed based on events,
fans still desire control over when and what data should be displayed.
% Thus, we implemented keyboard-based interaction 
% to turn on or off a specific visualization during live game viewing.
% Each visualization was mapped to a key, i.e., ``O'' key for the Offense Trajectory.
During the user study, 
we applied the Wizard-of-Oz (WoZ) method~\cite{dahlback1993wizard,dow2005wizard} to allow fans to control the visualizations with voice commands, while the experimenter manually turned each visualization on and off.
% using the keyboard, e.g., pressing the ``D'' key for the Defense Form. 
The WoZ method is commonly used to evaluate complex, intelligent systems while reducing implementation effort~\cite{budzianowski2018multiwoz,palmeiro2018interaction,browne2019wizard}. 
Most importantly, the current speech recognition systems cannot meet the speed and accuracy requirements for fast-paced use cases, like sports.
We envision with the advance in speech recognition and natural language processing, a robust system will be available in the near future.
% Using voice commands allows for a natural interaction,
% during live game viewing for fans, 
% but the speed and accuracy of current speech recognition systems still has many challenges.
By using a WoZ method, we can ensure the consistency of user experiences without being hindered by current speech recognition systems. 
% and conduct the user study remotely with minimal interaction requirement from the users. 
% Thus, we implemented both keyboard and voice command to allow fans 
% to turn on or off a specific visualization during live game viewing.
% Each visualization was mapped to a command, i.e., ``O'' key and ``Offense'' voice command for the Offense Trajectory using keyword recognizer~\cite{keyword_recognizer}.
% We didn't implement mouse-based interactions since mouses are usually unavailable and counter-intuitive in a TV watching environment.
Nevertheless, 
while interaction techniques are not the focus of our study, 
we identified insights regarding users' interaction preferences as implications 
for future work in Sec.~\ref{sec:implications}.


% We leave a more comprehensive study of the interactions in such an environment for the furture work.



% Therefore, we chose voice-based interaction for users to control the system in the user study. Furthermore, we identified insights regarding users' interaction preferences as implications for future work in Sec.~\ref{sec:implications}.

==> [2022 VIS] Omnioculars/docs/6_user_study.tex <==
% !TEX root = ../main.tex

\section{User Study}
\label{sec:user-study}

We conducted a controlled user study with active basketball fans to evaluate the usefulness and user engagement of Omnioculars.

\subsection{Experiment Set-Up \& Participants}

To simulate the game contexts,
we chose a famous game between Golden State Warriors and Cleveland Cavaliers on Dec 25th, 2015. 
This Christmas game featured the best teams from the previous season's final, 
who faced each other in the championship again, 
and was selected as one of the best games by the NBA in the 2015-16 season.
All the required data, like event data, shot locations, and player zoned shot percentage,
is publicly available~\cite{kagglenba, espn2015, nbashotcharts, basketballref},
except for the tracking data. %and downloaded online
We could only obtain 2D tracking data of the ball and players~\cite{sportvu}.
To preserve the authenticity of the game viewing experience in our prototype, 
we manually annotated the vertical positions and polished the player model animations to reflect the game events as closely as possible.

For our study, we selected three video clips from the simulated game. 
Each clip consists of about 30 seconds with two to three plays, focusing on shooting, offense and defense performance, and the clutch time situation. 
We used two video clips in the first part of the user study and counter-balanced them for use as either training or study clip among participants. %were altered as training and study clip among the participants. 
We used the third clip, which contains the clutch time situation, for the second part of personalized game analysis. 
% To ensure the consistency of user experiences with voice commands, 
% we applied the Wizard-of-Oz method~\cite{dow2005wizard} during the user study. 
% The experimenter manually enables or disables each visualization based on the user's voice command.

We recruited 16 participants through the university mailing list after an initial screening of their fandom levels (P1-16; M = 13, F = 3; Age: 18 - 45). We targeted active fans who reported watching games at least once a week during the game season and were interested in looking up data during the game. 
% Participants ranged in age from 18 to 45 years (3 females and 13 males). 
Four identified as casual fans, seven as engaged fans, and five as die-hard fans.
We conducted the user study over Zoom, which took one hour per participant to complete. 
We compensated each participant with a \$20 gift card.
% goal of the user study
%We designed a controlled user study to evaluate the helpfulness and engagement of Omnioculars with targeted active basketball fans in two parts. 

% \zt{this part is repetitive to Sec.6.2?}
% Using the think-aloud method on simulated game clips, we first assessed the understandability and insights generated by fans with five embedded visualizations, respectively, including Shot Label, Offense Trajectory, Defense Form, Shot Chart, and Team Panel.  
% The user rated and commented on the useful contexts supported by each visualization in the game clip. This allows us to quantify each visualization's usability and usefulness, and provide empirical evidence to verify our design framework. 
% % 
% In the second part, we asked participants to freely explore different visualization combinations using voice commands, and collect their subjective feedback and interaction strategy to characterize their game understanding and engagement with Omnioculars. This allows us to evaluate the usefulness and engagement of the interactive embedded visual game analysis system as a whole, and identify opportunities and limitations for future work.
% To ensure the consistency of user experiences with voice commands, we applied the Wizard-of-Oz method~\cite{dow2005wizard} during the user study. The experimenter manually enables or disables each visualization based on the user's command.

% Set up: remote , sharing through zoom
% part 1: five visualization with training
% part 2: remote control of the embedded vis in the video 

% \textbf{Player tracking data.} 
% We collected  ball and player tracking data from SportVU~\cite{sportvu}. 
% % https://paperswithcode.com/dataset/nba-sportvu
% The available data set contains NBA regular-season games for the 2015-16 season. 
% Due to the limited tracking data, we could only obtain 2D positions of the ball and players. 
% \textbf{Play-by-play data.} 
%  We obtained the data set on Kaggle~\cite{kagglenba}, which was originally from Basketball-Reference.
% % https://www.kaggle.com/schmadam97/nba-playbyplay-data-20182019
% \textbf{Box score data \& shot location.} 
% We obtained box score data and game shot chart data from ESPN website~\cite{espn2015}.
% % https://www.espn.com/nba/playbyplay/_/gameId/400828325
% \textbf{Player zoned shot percentage \& League average.} 
% We obtained players' shot chart from querying individual records on NBA Shot Charts website~\cite{nbashotcharts} 
% % http://nbashotcharts.com/home
% and league average data from Basketball-Reference~\cite{basketballref}.
% % https://www.basketball-reference.com/leagues/NBA_2016.html


% https://www.espn.com/nba/story/_/id/13426016/best-games-2015-16-nba-schedule

% We implemented this game in our Omnioculars prototype for two reasons. 
% First, 2015-16 is the most recent season with open-sourced player tracking data. 
% Second, choosing a famous and memorable game allows us to better communicate with our target basketball fans since all of them remember the rivalry between Warriors and Cavaliers. 



\subsection{Design \& Procedures}
% We recruited 16 participants through the university mailing list after an initial screening of their fandom levels. We targeted active fans who report having watched games at least once a week in the game season and are interested in looking up data during the game. Participants ranged in age from 18 to 45 years (3 females and 13 males). Four identified as casual fans, seven engaged fans, and five die-hard fans.

The study had two parts. The first part focused on assessing the understandability and usefulness of the five embedded visualizations (\ShotLabel{}, \Offense{}, \Defense{}, \ShotChart{}, and \TeamPanel{}). After being introduced to the study and filling out a consent form, the participants went through five rounds, one for each visualization condition. At the beginning of each round, we introduced each visualization design and led participants through a training task to think aloud their game insights from analyzing the embedded visualization in a game clip. After they were familiar with the visualization technique, they completed one study task of analyzing the game with the embedded visualization on another game clip. The participants were asked to rate and comment on the useful contexts supported by each visualization. 
% 
The second part focused on the usefulness and engagement of the Omnioculars system as a whole. We asked participants to freely explore different visualization combinations using voice commands. Participants first completed a training task to analyze a game clip with interactive visualizations using voice commands. They then completed one study task of thinking aloud their game insights from using interactive visualizations in another game clip. We asked them to rate the usefulness and engagement of the overall Omnioculars system and to comment on their strategy of using different visualizations to generate game insights. At the end of the study, participants filled out a post-study questionnaire. 
% The participants were first introduced to the study goal and procedures and filled out a consent form. Then, they practiced the think-aloud method to elaborate their game insights on a training clip without any embedded visualization. In Part 1, the participants went through five rounds, one for each embedded visualization condition. At the beginning of each round, the instructor first introduced the visualization design and explained how to read them. The users were led through a training task to get familiar with each visualization technique. Then, the users completed one study task by thinking aloud their game insights from analyzing the embedded visualization in a game clip. The users were asked to rate the visualization and provide feedback after the task. 
% In Part 2, the participants were introduced to the voice commands to control the visualizations in the video and went through a training task to get familiar with the
% interaction. Then, the users completed one study task by using interactive visualization to analyze game insights in a game clip. They were asked to rate the usefulness and engagement of the overall Omnioculars tool and commented on their strategy of using different visualization to generate game insights. At the end of the study, participants filled out a post-study questionnaire. 
% The whole study took one hour to complete, and each participant was compensated with a \$20 gift card.



\subsection{Measures}
\textbf{Part 1.} For each embedded visualization condition, we collected the subjective ratings on a 7-point Likert scale \re{from low to high}, including understandability, usefulness, engagement, and novelty. We also collected qualitative feedback, including the game insights generated by the participants while watching the game clip with each visualization, and the oral feedback about the contexts in which they found each visualization helpful and interesting to use.

\para{Part 2.} We collected subjective ratings on the usefulness and engagement of Omnioculars, where we derived our questions from prior work~\cite{o2010development}, including \textit{``It was helpful''}, \textit{``It was fun''}, \textit{``I felt in control''}, \textit{``I felt encouraged''}, and \textit{``I am likely''} to use Omnioculars to consume the desired game data in-game. We collected qualitative feedback of participants' strategy of using different visualizations and the strengths, weaknesses, and suggestions for Omnioculars in a post-study questionnaire. 

\para{Qualitative Analysis.}
% Two authors color-coded the responses from 16 participants, and then used the affinity diagram to categorize the user feedback and derive common themes across all participants.
Participants' responses were analyzed by two authors using affinity mapping. In Part 1, we derived primary use cases for each visualization by grouping similar user insights. In Part 2, we categorized user strategy in personalizing the visualizations and the subsequent insights. The grouping results are shown in Appendix D. 


==> [2022 VIS] Omnioculars/docs/7_results.tex <==
% !TEX root = ../main.tex


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/Rating2.png}
    \vspace{-5mm}
    \caption{User study results. In Part 1, (a) participants rated all five embedded visualizations to be easy to understand, helpful, fun to use, and novel ways to present game data (Mdn $\geq 5$). In Part 2, (b) participants confirmed the usefulness and engagement of Omnioculars, were likely to use it in future games (Mdn$=7$), and perceived the simulated game as comparable to an actual game (Mdn$=6$). (c) Participants used different visualizations to perform game analysis.
    % in Part 2 of the user study \jb{a bit unclear what (c) means}. \jb{was a and b for part 1 of the user study? clarify}
    } 
    \label{fig:rating}
    \vspace{-4mm}
\end{figure}


\section{Results \& Discussion}
\label{sec:results}
% updated to all 16 participants' qualitative analysis
% include at least one quote from each participant
We present the user study results on how well embedded visualizations help users enhance game understanding and engagement,
and discuss the design implications for future interactive game viewing.

\subsection{What Game Insights Do Fans Generate with Each Embedded Visualization?}
In Part 1 of our study, participants provided their game insights while using each embedded visualization, and commented on helpful use cases. We discuss user subjective ratings and findings below. A detailed categorization of user comments can be found in Appendix D. 
% \jb{maybe more info to affinity mapping, ref to fig 5a and shorten text of 7.1, refer to supplemental material for user comments?}

% 
\para{Five embedded visualizations were perceived to be useful and novel}. 
In Fig.~\ref{fig:rating}a, participants rated each visualization from 1 (low) to 7 (high) on Q1) easy to understand, Q2) helpful, Q3) fun to use, and Q4) novel ways to present game data. The majority rated all five embedded visualizations positively ($>4$) in usefulness and engagement, \re{reporting that they were} easy to understand ($\geq $88\%), helpful ($\geq $75\%), and fun ($\geq $69\%). For novelty, Shot Label was rated novel by 94\% of the participants, Offense, Defense, and Shot Chart by  75\%, and Team Panel by 56\%.

% Shot Label - game insights, when is useful, then discuss some comments
\para{Participants used the \ShotLabel{} to evaluate individual player performance and player decisions}. Participants used color on the dynamic label to evaluate players' shot performance, \textit{``Sean Livingston is very low from the 3-point line (P2)''}. %, \textit{``It’s interesting to see how the percentages change between good scorers and bad ones (P13)''}. 
% \textit{``To know if a player shoots better/worse than league average is very interesting. (P11)''}. 
% Some participants tried to use the shot percentages of the players to predict the next plays, e.g., \textit{``It’s interesting to try predicting what play is going to happen next while visualizing the ball handler's shooting skills. (P14)''}. 
Furthermore, some participants contemplated the player's decision-making, \textit{``When I see Lebron drives, the color changed drastically, so I get that why he did not make the three-point shots and tried to take the drive. (P1)''}. Overall, participants found the Shot Label most helpful to focus on player and ball movement, and after shooting.
% \textit{``immediate visual feedback after the pass (P3)''}, and after shooting, \textit{``to see whether he made the right decision based on his average (P15)''}. 

% Offense
\para{Participants used the \Offense{} to spot the shot opportunity and team strategy}. Participants used the circle underneath the players to evaluate the shot opportunity, 
% e.g., \textit{``I used the size to spot the shot opportunity and the player position (P6)''} \jb{can we remove this prior user comment? it is not very insightful}, 
% and identify team strategy, 
\textit{``They passed to people who had more space, or a larger circle, at the time (P7)''}, and the trails to read the team strategy, %\textit{``I focus more on the trail to identify the movement (P8)''} and 
\textit{``Like this run, [trails] help me understand the team better, not just the player individually (P1)''}. 
Participants found the Offense Trajectory most useful when they focused on team offense strategy  
% \textit{``To understand how players create shot opportunity (P4)''}\jb{remove}, 
and following offense during the transition, \textit{``
% During transition, the distance to the defenders is 
When defense changes quickly, 
seeing opportunity arose when somebody was breaking away to the basket or slipped away from the defenders is helpful (P3)''}.

% Defense
\para{Participants used the \Defense{} to track defense changes and strategy}. Participants used the color of the circle underneath the players to identify defenders. 
% e.g., \textit{``I could see when the defensive player becomes effective with color changing from blue to dark blue (P4)''}.
% \jb{rm}. 
% and \textit{``Lebron gets the ball and crosses multiple defenders. I can see the color highlighting the defenders (P9)''}. 
They also observed the defense strategy,
% \textit{``Interesting to see and predict who will be the ball defender. (P11)''}, 
\textit{``The shaded area between the defenders shows how the defense blocked the paint area to get the rebound (P6)''}. Participants found the Defense Form most useful when they wanted to track defense changes during a switch or transition 
% \textit{``Coming out of the transition into half court offense (P3)''} \jb{rm} or
% \textit{``during the switching, when there is a mismatch or double guarding (P1)''}\jb{rm}, 
and to identify the defense strategy. 
% \textit{``When a team is playing zone defense (P16)''}\jb{rm} or \textit{``to track the defense strategy of primary ball handler, and identify number of defenders (P10)''}\jb{rm}.\jb{imho, too many comments}
% e.g., \textit{``when it is a lot going on, you can kind of squint and see how many defenders are near the ball (P2)''}.

% Shot chart
\para{Participants used the \ShotChart{} to examine the overall shot performance and shot decisions}. Participants used the heat map and virtual balls on the court to evaluate the player's shot performance. 
% e.g., \textit{``Lebron has many shot attempts (P5)''}.
% , \textit{``I didn't realize Lebron is so much better in the paint. (P3)''}\jb{rm}. 
They also derived insights on players' shot decisions 
% e.g., \textit{``Most of Lebron's shots are dunks (P2)''}\jb{rm}, 
and on how players compare between each other, \textit{``It’s interesting to see the chart differences between shooters and role players. (P13)''}. Participants found the Shot Chart most useful to understand shot selection, \textit{``When there were lots of shots from a particular area, to understand if they were high percentages shot or not (P11)''}, and to evaluate players' shot performance immediately, 
% \textit{``right after a shot and before another play happens (P12)''}\jb{rm} and 
\textit{``to understand someone’s performance and contribution, especially with players I don’t know (P14)''}.
% \textit{``Show for the shots if I'm not as familiar with the player, especially for the opposite team to understand the person who just made the shot (P2)''}.

% Team Panel
\para{Participants used the \TeamPanel{} to compare team performance}. Participants used the team panel to check on game stats. 
% e.g., \textit{``I look quickly to track score change. (P6)''} \jb{rm}. 
They also derived game insights from the color encoding, \textit{``Interesting to see both teams had lower shot percentages compared to the league average (P10)''}. 
% \textit{``Cav is trying to use their advantage to get free throws (P7)''}\jb{rm}. 
Participants found the Team Panel most useful to follow the team's progress throughout the game 
% \textit{``Information is quite helpful to have there anytime during the game (P12)''} 
% and \textit{``Not a specific time, but throughout the game to see the stats an compare them it’s useful (P13)''} \jb{rm},
and to analyze areas of focus, \textit{``When the game score is close, I can see the key factors to evaluate and predict the outcome (P8)''}.

% discuss
\para{Overall, each embedded visualization provides helpful data on different game aspects for the participants}. The obtained insights and identified use cases aligned with our design contexts. 
While individual needs and knowledge levels vary, all participants were able to generate different game insights from each visualization.
% they perceived each visualization to be easy to understand, helpful and fun to use while watching the game, and a novel way to present game data with high satisfaction, as shown in Fig.~\ref{fig:rating}(a). 




\subsection{How Do Fans Personalize Omnioculars to Enhance Game Understanding and Engagement?}
% - how do fans use the combination of vis to generate game insights?
In Part 2, participants interacted with Omnioculars to use different visualizations to generate game insights. We were interested to see how they combined or altered visualizations during the game, how their individual preferences impacted their strategies, and how the selected embedded visualizations helped users generate game insights. 

% how they combine & alter vis during the game
\para{Participants used various combinations of the different visualizations.}
%Different visualizations were used at different frequencies, as shown in Fig.~\ref{fig:rating}(c). 
Fig.~\ref{fig:rating}c shows the usage patterns of the five visualizations for each participant (the amount of time a certain visualization was displayed).
% During the 30-second game clip, Shot Label was used the most, and Shot Chart and Team Panel were used less frequently. The usage frequency reflected the use cases of each design, where Shot Label, Offense and Defense were designed to be used continuously to track dynamic player performance, while Shot Chart and Team Panel were used occasionally at discrete game moments. 
On the individual level, each participant chose different visualization combinations and focused on different aspects of the game. Six participants used all five visualizations, and all users used at least three. Each visualization was used frequently ($>33\%$) by several users each, i.e., Shot Label (by 13 users), Offense (9), Defense (9), Shot Chart (4), and Team Panel (7).  


\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{images/strategy.png}
  \vspace{-6.5mm}
  \caption{(a) and (b) show personalized visualizations configured by different users during the user study.}
  \vspace{-6.5mm}
  \label{fig:strategy}
\end{figure}

% how individual preference impact their strategies
\para{Participants developed different strategies to engage with the visualizations based on individual preferences and their game focus.}
We observed two primary user strategies. 
The first strategy was \textbf{``configure a fixed set''}, \re{which was used} by eight participants. These users first identified their preferred combination of visualizations and used this fixed set throughout the game clip. They hoped to access personalized visualizations to facilitate game analysis without having to actively control them. Among them, we identified two styles of rationales, analytic-driven and experience-driven. Analytic-driven users decided the visualization set based on their game analysis needs.
For example, P6 used Team Panel, Defense, Shot Label all together (Fig.~\ref{fig:strategy}a), and explained that \textit{``these help me focus on why they are playing this way, see if they switch or not, and track the shot percentage''}. On the other hand, P3 used Team Panel at first, 
% then turned it off 
and used Shot Label and Shot Chart together for the rest of the game clip. P3 explained that \textit{``I wanted the team panel first to get an idea of how things were going thus far.
% and I probably wouldn't have turned it on again. 
Shot Label and Shot Chart are very useful for seeing current instant threats by the ball handler. I also appreciated seeing whether a player was hot compared to their average''}. 
Experience-driven users chose the visualizations based on engagement. For example, P2 wanted to start with everything on because \textit{``it's already such a fast-paced sport that I liked just having them on.''}
P15 used Shot Label, Defense, and Shot Chart together because \textit{``they are very fun to use and watch''} (Fig.~\ref{fig:teaser}).
% 
The second strategy was \textbf{``alter based on context''} \re{adopted} by eight users. 
Participants selected visualizations based on their needs, which varied based on the current game context.
%The visualizations were actively selected based on the users' needs at the moment and varied based on game contexts. 
For example, P5 explained that \textit{``during the clutch time, I'll look at team panel. When the game is not as intense, I will look at defense and offense''}. Some participants selected visualizations based on the team they support, \textit{``If I'm watching a game of a team I am rooting for, I focus on the visualization on that (offense/defense vis when the team is attacking/defending)''}. Other fans showed more flexibility, \textit{``I first use Offense and Defense to understand the team drills} (Fig.~\ref{fig:strategy}b). \textit{When I am familiar with them, I'll use Shot Label to evaluate if the shot selection is reasonable (P9)''}. 
% or \textit{``I would use the visualizations to see how my team is playing (P13)''}. 

\para{Embedded visualizations help participants derive insights.} % into the game aspects of their focus.}
When asked about the game insights they obtained with Omnioculars, participants focused on distinct aspects, such as \textit{identify} player movement and decision making, \textit{compare} player's in-game stats, or \textit{summarize} game performance. These goals align with the data and tasks we identified in Sec.~\ref{ssec:data_context}.
For example, P2 used the Offense Trajectory to focus on player decisions, \textit{``when he just passed, I think it's cool to see that there's not really open shots as there's no big yellow circle anywhere''}. P3 evaluated player's shooting with the Shot Label, stating \textit{``it's so interesting to see the shot percentage climb up as they drive to the basket''}.
Additionally, 
P1 used the Team Panel to derive a game summary, \textit{``We are doing really well in the assist and block, wow that's unexpected. The turnover is a problem, but if you have more assists, you're supposed to have more turnovers. I think that's acceptable.''}. 


% Participants also expressed excitement and engagement in finding the game insights.
% 
% As shown in Fig.~\ref{fig:strategy}c, each participant utilized different combinations of visualizations to help them generate game insights. This reflects the distinct focus of different audiences.


% \para{\re{Overall, Omnioculars was rated helpful and fun for game understanding and engagement}}, as shown in Fig.~\ref{fig:rating}b.

% \para{Overall, participants were highly satisfied with Omnioculars in helping them understand and engage in the game}. 
% As shown in Fig.~\ref{fig:rating}b, 
% participants found Omnioculars helpful and fun (100\%), %
% % e.g., \textit{``It helps me engage in the game (P1)''}, \textit{``It sticks with the movements of the players so it's easy to follow (P11)''}. 
% % In addition, they 
% felt in control of their game viewing experience (94\%) and encouraged to consume data during the game (100\%).
% % , e.g., \textit{``I like being in control to see what I wanted to see (P13)''}, 
% % \textit{``I like it's the same information that somebody might tell you, but I think it's better to see it (P2)''}.
% They also expressed high interest in using Omnioculars in live games, if available  (100\%). 

% We discussed further implications for simulating real-world events in the virtual environment in Sec.~\ref{sec:game-simulation}.




\subsection{Implications for Future Interactive Game Viewing}
\label{sec:implications}
% discuss findings from user study - 
% improvement / suggestions for future design

% - the depth of game insights obtained from the visualization vary by fandom level
% (more advanced and passionate fans can gain more out of the visualization)

\para{Flexible embedded visualization design is important to enable a customized experience.}
A key finding is that individual needs for data and desired interaction levels vary. Based on the user's preferences and basketball experience, some people felt a visualization was distracting and overwhelming, while others felt the same visualization helped them see the data more easily. For example, the trails in the Offense Trajectory visualization were perceived useful to evaluate offense strategy by some die-hard fans, \textit{``The trails are great to see the players' strategy when the players are closer, like pick-and-roll. It makes it easier to see the tactics (P9)''}. 
However, other fans felt they only focused on the circles to identify the shot opportunity and did not utilize the trails, \textit{``I just feel like it's too much information to follow. (P2)''}. %shorten, \textit{``I didn't look much at the trajectories because I wasn't very interested in every players' movement (P12)''}. 
% We found that advanced and data-savvy fans also tend to gain more insights on the strategic level, such as player decision or team strategy, and more casual fans focus on the execution level, such as track defenders or shot opportunity. These findings highlight the need to provide further customization of the visualizations.
A recommended solution is to decouple the individual components of a visualization, such as separating the trail and circle in the Offense Trajectory visualization, or the heat map and player panel in the Shot Chart visualization. As participants focus on a range of goals based on their preferences, allowing them to select and mix from independent visual components can best fulfill their individual needs. 

\vspace{-0.8mm}
\para{Embedded sports visualizations are still underexplored.}
%\noindent\textbf{A large underexplored space for embedded sport visualization design and subjective dimensions matter.}
We iterated our designs with targeted users, and we believe they are the most suitable in the scope of this project.
However, we also believe there is a need for more refined embedded visualizations targeting specific tasks and contexts based on our proposed design framework.
Additionally, designing embedded sports visualizations not only requires consideration for objective dimensions such as perceptual effectiveness, but also for subjective dimensions, such as engagement, which plays a more vital role compared to traditional visualization design.

\vspace{-0.5mm}
\para{Expressive interactions allow users to go beyond a passive viewing experience.}
We used voice commands as the interaction mechanism for our study, as we believe, with overwhelming choices, it can best articulate the user's intention~\cite{srinivasan2020ask,srinivasan2021collecting,Shen2022TowardsNL}, especially in fast-paced sports watching. 
Participants had different opinions about the provided interactions:
% In terms of interaction with the system, 
a few participants preferred to have a certain level of default behaviors, \textit{``I wish Shot Chart would turn on automatically for a few seconds after shots % and then turn off automatically 
(P2)''} and \textit{``I feel like it would be a hassle to be turning it on and off and on and off (P3)''}, while others enjoyed having interaction, 
% \textit{``I like interaction with the system the most (P4)''}, particularly the voice commands in the study, 
\textit{``I liked the voice activated part of it, very useful to follow the game and still visualize what I wanted (P11)''}. To this end, we suggest an interaction approach that would allow users to configure default settings based on their game focus on desired data. % targeted game contexts and desired data. 
Future work can explore interaction design space in the spectrum from manual to automatic and train personalized AI models to support semi-automatic interactions. 
In terms of functionality, we only allowed simple interactions to toggle visualizations on and off, mainly considering the fast-paced nature of sports. However, more complicated interactions could be required (check the average stats of three players). 
% Voice command can still be a great candidate, but 
Future research can explore other interactions to support in-game data analysis.


\para{A systematic evaluation of human perception and attention could shape embedded visualization design.}
Participants highlighted the advantages of our embedded visualization design for game viewing, including providing immediate feedback, being easily accessible while watching the game video, and alleviating mental load.
For example, the Shot Label visualization provides \textit{``immediate visual feedback after the pass. I've seen the color flip from red to blue to immediately know that (P3)''}. With Team Panel sitting next to the court, \textit{``I can look at it, for as long as I need to and then switch over to looking at what's happening now (P2)''}.
The visualization can help fans focus on the ball, \textit{``I could still be watching the ball, but out of the corner of my eye could see whether or not they had options (P12)''}. 
As the first step towards understanding the use of embedded visualization in sports, our work aims to provide proof-of-concept results for the design space and its effectiveness. 
As a result, we did not systematically evaluate these potential advantages in our study.
We believe, as future work, obtaining empirical knowledge of these effects can largely facilitate the development of embedded sports visualization. 
% While these advantages were not evaluated in our study, understanding the impact of embedded visualization on human perception and attention can be an interesting future work direction.


\para{\re{Future broadcasting with interactive embedded visualizations.}}
\re{
% Our simulated game environment built upon existing player tracking data and live game stats provided by official broadcasters (SportVU, ESPN).
In current live streams of games, camera angles may change and cut off the scene. Without access to camera configurations and the complete video footage, embedding visualizations into videos accurately can be difficult. 
However, broadcasters already collect all the required information, such as tracking data and the full video footage. Therefore, we believe our design framework and visualizations can be adopted and extended to augment actual live games by the broadcasters, or by researchers once the data are made available. Similar to our envisioning direction, a few personalizations are already offered by the NBA, such as customized viewing angles with the NBA League Pass} \cite{nbaleaguepass} 
\re{and augmented visual overlays on the live game view by CourtVision} \cite{clipperscourtvision}.

\para{Beyond-the-screen game viewing.}
% \noindent\textbf{In-person augmented game viewing.}
Many people prefer watching games in person to experience the live atmosphere.
Unlike watching a game through digital devices with visual effects, it is challenging to overlay extra information on a physical court.
Fortunately, with recent advances in augmented reality (AR), it is now possible to embed digital graphics into the physical world.
We believe that using AR to embed visualizations into an in-person game will enhance the game viewing experience, and help spectators make sense of the real-time game data.
We also believe our results can be largely generalized to an AR in-person game viewing scenario, as we designed and implemented our system in a 3D environment (Unity3D).
However, using our designs in AR still differs from a flat screen and we need to consider: the effect of stereoscopy vision and depth perception; the limited field of view (FoV) in current AR devices; and the ability to freely change viewing direction so that physical and digital objects can be out-of-view.
In the future, we plan to adapt our current system to AR (by adding out-of-view notifications and by simplifying visualization designs based on the FoV) and to evaluate its effectiveness.



% - use of color is very important, people mentioned multiple times they think the color was cool, when the color changes it catches their eyes, etc.



% - Fundamentally, we want to provide ideas/guidance for future visualization and interaction designs.

% interaction
% - do people want interactions at all? If so, how much and what are those?

% - what are the fundamental interactions we need? E.g., fast player selection and more?

% - how to make the current visualizations interactive? I.e., not just show/hide. It is also important to know what the users can interact with the tested visualizations in an ideal world.

% - is voice command the best way? What are the other alternatives? 

% - Customization is important, and can only be achieved by interactions. Semi-automatic method seems to be the most practical and ideal. It can be possible to train personalized AI model to achieve full-automatic visual effects?

% visualization design
% - what are the extra visualizations/information mentioned by the participants?


\subsection{Simulating Basketball Games in a Virtual Environment}
\label{sec:game-simulation}
% 94\% of participants considered the game insights from the simulated game comparable to an actual game (Mdn = 6). 
% Due to data and technical limitation, our simulations did not recreate detailed player animation like a fake or a dunk action, which could cause some confusion, e.g., \textit{``Some simulation part looks confusing, like a player spinning around in the same position (P7)''}. However, all participants were able to observe game actions and obtain meaningful insights throughout the study. \zt{flesh out this paragraph with more user study results}
% 

Our study shows that simulation can be a promising solution to ease the development and evaluation 
of visualizations embedded in physical contexts. 94\% of all users considered game insights derived from the simulated game comparable to an actual game (Fig.~\ref{fig:rating}b). 
Compared to traditional visualizations presented in digital environments,
embedded and situated visualizations presented in physical contexts
are difficult to develop and evaluate 
due to the limited accessibility and controllability of the physical contexts.
Moreover, unlike web-based visualizations,
embedded and situated visualizations are inherently challenging to distribute, reproduce, and benchmark,
hindering the research progress in this emerging direction.
% - tradeoffs between actual game vs. simulation
% - potential benefits of this simulated context as a research method for immersive analytics research
By compromising a certain degree of fidelity,
simulation enables a highly accessible and controllable physical context that can be shared, reproduced, and compared universally,
significantly lowering the barrier to designing embedded or situated visualizations.
In recent years, thanks to the proliferation of low-cost VR devices,
many researchers~\cite{shimizu2019sports, tsai2020feasibility, tanaka2018scope, ye2020shuttlespace, chuTIVEEVisualExploration2022, DBLP:conf/uist/ChengY0SL21}
have leveraged VR to simulate real-world environments
in user-centered design studies.
We envision and advocate a standard simulation protocol for developing visualizations in physical contexts,
which may eventually facilitate the research of embedded and situated visualizations. 
% for designing, developing, and evaluating embedded or situated visualizations,
% which may eventually facilitates the research of embedded or situated visualizations. 

==> [2022 VIS] Omnioculars/docs/8_conclusion.tex <==
% !TEX root = ../main.tex

\section{Conclusion \& Future Work}
This study explored the design space of embedded visualization for basketball in-game data analysis. 
Through a user-centered design process, we presented a formative study of basketball fans' in-game data needs and proposed a context-driven design framework of four design elements --- \emph{Scenario}, \emph{Data}, \emph{Task}, and \emph{Embedded Vis}. We designed five embedded visualizations for five primary game contexts and developed Omnioculars, a prototype for personalized game viewing with embedded visualizations. 
Our evaluation results suggest that each embedded visualization provides helpful data on different game aspects, and fans developed different strategies to engage with visualizations based on their individual preferences and game focus with Omnioculars.


% , first, each embedded visualization provides helpful data on different game aspects for the participants. 
% Second, users developed different strategies to engage with visualizations based on their individual preferences and game focus.
% %Second, different strategies were developed to engage with visualizations based on individual preferences and game focuses. 
% Third, overall, participants were highly satisfied with Omnioculars in helping them understand and engage in the game.
%  
% For future work, we identified the necessity to allow customizable visual complexity and interaction with embedded sports visualizations based on individual preferences and knowledge levels. To this end, incorporating domain experts' knowledge and
% using ML models to specify game contexts and refine visualization designs are both promising directions.
% We also hope to build upon the current design framework to explore using embedded visualizations for immersive and situated in-game data analysis.
% 
For future work, we identified the necessity to allow customizable visual complexity and interaction with embedded sports visualizations based on individual preferences and knowledge levels. We also hope to build upon the current design framework to explore using embedded visualizations for immersive and situated in-game data analysis.

==> [2022 VIS] Omnioculars/docs/9_acknowledgements.tex <==
% !TEX root = ../main.tex

%% if specified like this the section will be committed in review mode
\scriptsize
\acknowledgments{This work is
supported by NSF grants III-2107328 and IIS-1901030.
We thank Hans H., Joan C., Harvey H., Ahmed S., Nhan H., and Max M. for their time. }

==> [2022 VIS] Omnioculars/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

